Simultaneously Approximating All Norms for Massively Parallel Correlation Clustering

We revisit the simultaneous approximation model for the correlation clustering problem introduced by Davies, Moseley, and Newman[DMN24]. The objective is to find a clustering that minimizes given norms of the disagreement vector over all vertices. We present an efficient algorithm that produces a clustering that is simultaneously a $63.3$-approximation for all monotone symmetric norms. This significantly improves upon the previous approximation ratio of $6348$ due to Davies, Moseley, and Newman[DMN24], which works only for $\ell_p$-norms. To achieve this result, we first reduce the problem to approximating all top-$k$ norms simultaneously, using the connection between monotone symmetric norms and top-$k$ norms established by Chakrabarty and Swamy [CS19]. Then we develop a novel procedure that constructs a $12.66$-approximate fractional clustering for all top-$k$ norms. Our $63.3$-approximation ratio is obtained by combining this with the $5$-approximate rounding algorithm by Kalhan, Makarychev, and Zhou[KMZ19]. We then demonstrate that with a loss of $\epsilon$ in the approximation ratio, the algorithm can be adapted to run in nearly linear time and in the MPC (massively parallel computation) model with poly-logarithmic number of rounds. By allowing a further trade-off in the approximation ratio to $(359+\epsilon)$, the number of MPC rounds can be reduced to a constant.

==> not-used/_EdgeDeletion.tex <==


In this section, we analyze two approaches to convert $+$ edge into $-$ edge. Thus, we can get some properties of the new graph, e.g., each vertex in a $+$ connected component has a similar $+$ degree. \textbf{Note that we are currently only using one of these two approaches at a time}.

\begin{definition}
Here are the definitions of the two approaches:

\textbf{Approach 1.} $\forall (u,v) \in E^+$, assume without loss of generality $d(v) \ge d(u)$, if $d(v) \ge \alpha \cdot d(u)$, we convert $(u,v)$ into $-$ edge.

\textbf{Approach 2.} $\forall (u,v) \in E^+$, if $|N(u) \Delta N(v)|\ge \beta \cdot \max\{N(u), N(v)\}$, we convert $(u,v)$ into $-$ edge.
\end{definition}

\begin{lemma}
For any clustering $\mathcal{C}$ and any $(u,v)$ converted in \textbf{Approach 1} or \textbf{Approach 2} that is not cut ($u,v$ are in the same cluster) in $\mathcal{C}$, we have $\max\{d(u), d(v)\} \le O(1) \cdot (y_\mathcal{C}(u) + y_\mathcal{C}(v))$.
\end{lemma}

\begin{proof}
For any $(u,v)$ converted in \textbf{Approach 1} that is not cut in $\mathcal{C}$, we assume $d(v) \ge d(u)$, then $d(v) = \alpha \cdot d(u) + \delta, (\delta \ge 0)$.
So, there are at least $(\alpha - 1)\cdot d(u) + \delta$ vertices, each of them satisfy that $w\in V$, $(u,w)$ is $-$ edge and $(v,w)$ is $+$ edge, one of $(u,w)$ or $(v,w)$ is a disagreement and contribute to one of $y_\mathcal{C}(u)$ or $y_\mathcal{C}(v)$.
Then we have $\frac{\alpha -1}{\alpha} \cdot \max\{d(u), d(v)\} \le \frac{\alpha -1}{\alpha} \cdot  d(v) \le (\alpha - 1)\cdot d(u) + \delta \le |N(u) \Delta N(v)| \le y_\mathcal{C}(u)+y_\mathcal{C}(v)$. Therefore, $\max\{d(u), d(v)\} \le \frac{\alpha}{\alpha-1} \cdot (y_\mathcal{C}(u)+y_\mathcal{C}(v))$. 

For any $(u,v)$ converted in \textbf{Approach 2} that is not cut in $\mathcal{C}$, $\max\{d(u),d(v)\}\le \frac{1}{\beta} \cdot |N(u) \Delta N(v)| \le \frac{1}{\beta} \cdot (y_\mathcal{C}(u)+y_\mathcal{C}(v))$.
\end{proof}

\begin{lemma}
For a given instance $G$, any clustering $\mathcal{C}$, any integer $k$ (s.t. $1\le k\le n$),  any subset $U \subset V$ such that $|U| = k$. Let the number of edges converted by \textbf{Approach 1} or \textbf{Approach 2} incident to $u_i \in U$ that are not cut in $\mathcal{C}$ to be $\varphi(u_i)$. Then, $\sum_{u_i \in U} \varphi(u_i)$ is at most $O(1) \cdot \mathbf{OBJ}(G,k,\mathcal{C})$.
\end{lemma}

\begin{proof}
First, let the set $U'$ be the set of vertices $u_i\in U$ that satisfy $\varphi(u_i)>0$, i.e. there exists an edge $(u_i,v)$ that contributes to $\varphi(u_i)$. Let the $k$ vertices with the largest disagreement values to be $w_1,w_2,w_3,...,w_k$, which form the set $W$, and assume we have $y(w_1)\ge y(w_2)\ge y(w_3)\ge ...\ge y(w_k) = Y$. Then $\sum_{w_i\in W} y(w_i) = \mathbf{OBJ}(G,k,\mathcal{C})$. Note that in the analysis we will use \textbf{Approach 1} and the proof of \textbf{Approach 2} is the same.

To begin our analyze, we divide the number of edges converted into two parts. For $\varphi(u)>0$, if the converted edge $(u,v)$ has $u\not\in W$ and $v\not\in W$, then it will be counted in $\varphi_1(u)$, otherwise it will be counted in $\varphi_2(u)$. Then, $\sum_{u_i \in U} \varphi(u_i) = \sum_{u_i \in U'} \varphi(u_i) = \sum_{u_i \in U'}
 \varphi_1(u_i) + \sum_{u_i \in U'} \varphi_2(u_i)$

For $\varphi_1$, we have
\begin{align*}
    \quad \sum_{u_i \in U'} \varphi_1(u_i) &= \sum_{u_i \in U'\setminus W} \varphi_1(u_i)\\
    &\le \sum_{u_i \in U'\setminus W} d(u_i)\\
    &\le \sum_{u_i \in U'\setminus W} \frac{2\alpha}{\alpha-1}\cdot Y.
\end{align*}

For $\varphi_2$, let all edges that be counted in $\varphi_2$ form a set $\widehat{E}$, which with its endpoints form a subgraph $\widehat{G}$.

Notice that $\forall (u,v) \in \widehat{E}$, we have at least one of the endpoints in the set $W$. So we can bound $|\widehat{E}|$ by calculating the degree of some of the $w_i\in W$. 

We calculate a set $W'$ by:
\begin{itemize}
    \item Set $W'$ to be empty.
    \item For all $w_i\in W$, if there exists an edge $(w_i,v)\in \widehat{E}$ and $y(w_i)\ge y(v)$, add $w_i$ to $W'$.
\end{itemize}

Then we have
\begin{align*}
    \quad |\widehat{E}| &\le \sum_{w_i\in W'}  d(w_i)\\
    &\le \sum_{w_i\in W'} \frac{2\alpha}{\alpha-1}\cdot y(w_i)\\
    &\le \frac{2\alpha}{\alpha-1}\cdot \mathbf{OBJ}(G,k,\mathcal{C}).
\end{align*}

Still, we can notice that for an edge $(u,v)\in \widehat{E}$, if and only if $u\in U'\cap W$ and $v\in U'\cap W$, it will be counted twice in $\varphi_2$. Let the number of these edges to be $CT$.

We calculate a set $W''$ by:
\begin{itemize}
    \item Set $W''$ to be empty.
    \item For all $w_i\in W$, if there exists an edge $(w_i,v)\in \widehat{E}$, $w_i,v \in U'\cap W$ and $y(w_i)\ge y(v)$, add $w_i$ to $W''$.
\end{itemize}

Then we have
\begin{align*}
    \quad CT &\le \sum_{w_i\in W''}  d(w_i)\\
    &\le \sum_{w_i\in W''} \frac{2\alpha}{\alpha-1}\cdot y(w_i).
\end{align*}

Now, we can calculate $\varphi_2$:
\begin{align*}
    \quad \sum_{u_i \in U'} \varphi_2(u_i) &\le |\widehat{E}| + CT\\
    &\le \frac{2\alpha}{\alpha-1}\cdot \mathbf{OBJ}(G,k,\mathcal{C}) + \sum_{w_i\in W''} \frac{2\alpha}{\alpha-1}\cdot y(w_i).
\end{align*}

Observe that $|W''| + |U'\setminus W| \le |U'\cap W| + |U'\setminus W| = |U'| \le k = |W|$. Then we can finish our proof:
\begin{align*}
    \quad \sum_{u_i \in U} \varphi(u_i) &= \sum_{u_i \in U'} \varphi(u_i)\\
    &= \sum_{u_i \in U'} \varphi_1(u_i) + \sum_{u_i \in U'} \varphi_2(u_i)\\
    &\le \sum_{u_i \in U'\setminus W} \frac{2\alpha}{\alpha-1}\cdot Y + \frac{2\alpha}{\alpha-1}\cdot \mathbf{OBJ}(G,k,\mathcal{C}) + \sum_{w_i\in W''} \frac{2\alpha}{\alpha-1}\cdot y(w_i)\\
    &\le \frac{2\alpha}{\alpha-1}\cdot \mathbf{OBJ}(G,k,\mathcal{C}) + \sum_{w_i \in W} \frac{2\alpha}{\alpha-1}\cdot y(w_i)\\
    &\le \frac{4\alpha}{\alpha-1}\cdot \mathbf{OBJ}(G,k,\mathcal{C}).
\end{align*}

By using \textbf{Approach 2}, we have $\quad \sum_{u_i \in U} \varphi(u_i) \le \frac{4}{\beta}\cdot \mathbf{OBJ}(G,k,\mathcal{C})$.
\end{proof}

\begin{definition}
A vertex is \textbf{light} if it has lost more than $\lambda$-fraction of its $+$ edges using the \textbf{Approach 1} or \textbf{Approach 2}.
\end{definition}

\begin{lemma}
For a given instance $G$, any clustering $\mathcal{C}$ and any integer $k$ (s.t. $1\le k\le n$), we choose $k$ \textbf{different} vertices $u_1,u_2,u_3,...,u_k \in V$, which form the set $U$. \textbf{Convert all $+$ edges between two light vertices into $-$ edges.} Let the number of edges converted incident to $u_i \in U$ that are not cut in $\mathcal{C}$ to be $\phi(u_i)$. Then, $\sum_{u_i \in U} \phi(u_i)$ is at most $O(1) \cdot \mathbf{OBJ}(G,k,\mathcal{C})$.
\end{lemma}

\begin{proof}
First, let the set $U^*$ be the set of vertices $u_i\in U$ that satisfy $\phi(u_i)>0$, i.e. there exists an edge $(u_i,v)$ that contributes to $\phi(u_i)$, which means $u_i$ is a light vertex.

From the definition of light vertex, any light vertex $u\in U$ satisfy that $d(u)\le \frac{1}{\lambda}\cdot \varphi(u)$.

Then for \textbf{Approach 1} we have
\begin{align*}
    \quad \sum_{u_i \in U} \phi(u_i) &= \sum_{u_i \in U^*} \phi(u_i)\\
    &\le \sum_{u_i \in U^*} d(u_i)\\
    &\le \sum_{u_i \in U^*} \frac{1}{\lambda}\cdot \varphi(u_i)\\
    &\le \frac{1}{\lambda}\cdot \frac{4\alpha}{\alpha-1}\cdot \mathbf{OBJ}(G,k,\mathcal{C}).
\end{align*}

By using \textbf{Approach 2}, we have $\quad \sum_{u_i \in U} \phi(u_i) \le \frac{1}{\lambda}\cdot \frac{4}{\beta}\cdot \mathbf{OBJ}(G,k,\mathcal{C})$.

\end{proof}

==> not-used/_GeneralCases.tex <==


In this case, we can define $x_{uv} = 1 - \frac{|N^+(u) \cap N^+(v)|}{\max\{\Delta_u, \Delta_v\}}$, where $\Delta_u = |N^+(u)|$ is the $+$degree of $u$.  Then, for a $+$edge $uv$, its LP cost is $\frac{\Theta(1)}{\max\{\Delta_u, \Delta_v\}} \cdot \#(\text{bad triangles containing $u$ and $v$})$, where the constant is between $\frac12$ and $1$.  For a $-$edge $uv$, its LP cost is $\frac{1}{\max\{\Delta_u, \Delta_v\}}\cdot \#(\text{bad triangles containing $u$ and $v$})$.

==> not-used/_Notes-Shili-May82024.tex <==
	\section{Notes on 2024-05-07}
	
	Define the graph $H = (V, E_H)$ as follows, and the function $x \in [0, 1]^{{V \choose 2}}$ as follows:
	\begin{align*}
		E_H &= \Big\{uv \in E: \frac{d_u}{d_v} \in \big[\frac12, 2\big]\Big\}\\
		x_{uv} &= 1 - \frac{|N^H_u \cap N^H_v|}{\max\{d_u, d_v\}}, &\quad &\forall uv \in {V\choose 2}
	\end{align*}
	Nairen already proved that $x$ is a metric. To see this, think of the graph obtained from $H$ by adding $d_u - |N^H_u|$ dummy neighbors to each $u$. 
	
	Let $U$ be the set of $k$ vertices with the largest cost in the solution $x$. 
	
	For a triangle $uvw$ that is a $++-$ triangle in both $H$ and $G$, and $\{u, v, w\} \cap U \neq \emptyset$,  we define 
	$\alpha_{uvw} = \frac{1}{\max\{d_u, d_v, d_w\}}$. For all other triangles $uvw$, we define $\alpha_{uvw}= 0$.  Let  $\gamma_u = 1$ if $u \in U$, and $\gamma_u = \frac{|E_H(u, U)|}{d_u}$ otherwise.

	\begin{lemma}
		$(\alpha, \gamma)$ is valid up to an factor of $O(1)$.
	\end{lemma}	
	\begin{proof}
		$\sum_{u \in U} \gamma_u = k$, and $\sum_{u \notin U}\gamma_u \leq 2 \cdot \sum_{v \in U, u \notin U, uv \in E_H}\frac{1}{d_v} \leq 2k$. Therefore, $\sum_{u} \gamma_u \leq 3k$.  \medskip
		
		If $\{u, v\} \cap U \neq\emptyset$, we have 
		\begin{align*}
			\sum_{w}\alpha_{uvw} \leq O(1)  \cdot  \frac{|N^H_u \cup N^H_v|}{\max\{d_u, d_v\}} \leq O(1) \leq O(1) \cdot (\gamma_u + \gamma_v).
		\end{align*}
		Assume now $u, v \notin U$. Then 
		\begin{flalign*}
			&& \sum_{w \in U} \alpha_{uvw} \leq O(1) \cdot \frac{|E_H(\{u, v\}, U)|}{\max\{d_u, d_v\}} \leq O(1) \cdot \left( \frac{|E_H(u, U)|}{d_u} + \frac{|E_H|(v, U)}{d_v} \right) = O(1) (\gamma_u + \gamma_v). && \qedhere
		\end{flalign*}
	\end{proof}
	
	\begin{lemma}
		$\sum_{uv \in E:\{u, v\} \cap U \neq\emptyset}x_{uv} + \sum_{uv \notin E:\{u, v\} \cap U \neq\emptyset}(1 - x_{uv}) \leq O(1)\cdot (\text{DUAL}) + O(1) \cdot |d - d^H|_{\text{top-k}}$.
	\end{lemma}
	\begin{proof}
		For $uv \in E_H$ with $\{u, v\} \cap U \neq \emptyset$, we have
		\begin{align*}
			x_{uv} \leq \sum_{w} \alpha_{uvw} + \frac{(d_v - d^H_v)+ (d_u - d^H_u)}{\max\{d_u, d_v\}} \leq \sum_{w} \alpha_{uvw} + \frac{d_v - d^H_v}{d_v}+ \frac{d_u - d^H_u}{d_u}.
		\end{align*}
		Summing over all such edges $uv$, we have 
		\begin{align*}
			\sum_{uv \in E_H, \{u, v\}\cap U \neq \emptyset} x_{uv} \leq O(1)\cdot (\text{DUAL}) + O(1) \cdot |d - d^H|_{\text{top-k}}.
		\end{align*}
		Now, for $uv \notin E$ with $\{u, v\} \cap U \neq \emptyset$, we have
		\begin{align*}
			1 - x_{uv} = \frac{|N^H_u \cap N^H_v|}{\max\{d_u, d_v\}} \leq 2 \cdot \sum_w \alpha_{uvw}.
		\end{align*}
		Therefore, we have 
		\begin{align*}
			\sum_{uv \notin E: \{u, v\} \cap U \neq\emptyset}(1 - x_{uv}) \leq O(1) \cdot (\text{DUAL}).
		\end{align*}
	\end{proof}


==> not-used/_PrimalDual.tex <==

\numberwithin{equation}{section}
\renewcommand{\theequation}{LP \thesection.\arabic{equation}}

For the top-$k$ norm case for general $k$, the linear program relaxation is stated in ~\ref{lp:metric-lp}.

\begin{equation}\label{lp:metric-lp}
    \begin{aligned}
    \min_{x,z} \quad &z\\
    \mbox{s.t.} \quad &x_{uv}+x_{uw}\ge x_{vw} \quad &\forall u,v,w\in V\\
    &\overline{x_{uv}}=
        \begin{cases}
            x_{uv}, &uv\in E^+\\
            1-x_{uv}, &uv\in E^-
        \end{cases}\\
    &y_u=\sum_{v\in V} \overline{x_{uv}} & \forall u\in V\\
    & z\ge \sum_{u\in S}y_u & \forall S\subseteq V, |S|=k\\
    & x_{uv}\ge 0 & \forall u,v \in V.
    \end{aligned}
\end{equation}

When $uv\in E^+$, $uw\in E^+$, and $vw\in E^-$, we have $\overline{x_{uv}}+\overline{x_{uw}}+\overline{x_{uv}}\ge 1$. Let $\mathcal{T}$ be the set of bad triangles (i.e., triangles with exactly two positive edges and one negative edge), we can relax ~\ref{lp:metric-lp} into ~\ref{lp:badtriangle-lp}.

\begin{equation}\label{lp:badtriangle-lp}
    \begin{aligned}
    \min_{\overline{x},z} \quad &z\\
    \mbox{s.t.} \quad &\overline{x_{uv}}+\overline{x_{uw}}+\overline{x_{uv}}\ge 1 \quad &\forall uvw\in \mathcal{T}\\
    & z\ge \sum_{u,v \in V}|\{u,v\}\cap S|\cdot \overline{x_{uv}} & \forall S\subseteq V, |S|=k\\
    & \overline{x_{uv}}\ge 0, z\ge 0 & \forall u,v\in V.
    \end{aligned}
\end{equation}

% For a fixed set $S(S\subseteq V,|S|=k)$, let 
% $\gamma_u=
% \begin{cases}
%     1, \quad & u\in S\\
%     0, \quad & u\not\in S
% \end{cases}$, then we can get the primal given by ~\ref{lp:primal-fixedSet}, and its dual given by ~\ref{lp:dual-fixedSet}.
% 
% \begin{equation}\label{lp:primal-fixedSet}
%     \begin{aligned}
%     \min_{\overline{x}} \quad &\sum_{u,v\in V}(\gamma_u+\gamma_v)\cdot \overline{x_{uv}} \\
%     \mbox{s.t.} \quad &\overline{x_{uv}}+\overline{x_{uw}}+\overline{x_{uv}}\ge 1 \quad &\forall uvw\in \mathcal{T}\\
%     & \overline{x_{uv}}\ge 0
%     \end{aligned}
% \end{equation}
% 
% \begin{equation}\label{lp:dual-fixedSet}
%     \begin{aligned}
%     \max_{\alpha} \quad &\sum_{uvw \in \mathcal{T}}\alpha_{uvw} \\
%     \mbox{s.t.} \quad &\sum_{uvw \in \mathcal{T}}\alpha_{uvw}\le \gamma_u+\gamma_v \quad &\forall u,v\in V\\
%     \quad &\sum_{u} \gamma_u \leq k \\
%     &\alpha_{uvw}\ge 0, 0 \leq \gamma_u \leq 1
%     \end{aligned}
% \end{equation}
% 
% \begin{equation}\label{lp:dual-fixedSet2}
%     \begin{aligned}
%     \max_{\alpha} \quad &\sum_{uvw \in \mathcal{T}}\alpha_{uvw} \\
%     \mbox{s.t.} \quad &\sum_{uvw \in \mathcal{T}}\alpha_{uvw}\le \gamma_u+\gamma_v \quad &\forall u,v\in V\\
%     \quad &\gamma_u \leq \sum_{S \ni u, |S| = k}\tau_{S} &\forall u \in V \\
%     \quad &\sum_{|S| = k} \tau_{S} = 1 \\
%     &\alpha_{uvw}\ge 0
%     \end{aligned}
% \end{equation}

Let ~\ref{lp:badtriangle-lp} be the primal, and its dual given by ~\ref{lp:badtriangle-dual1}.

\begin{equation}\label{lp:badtriangle-dual1}
    \begin{aligned}
    \min_{\alpha,\beta} \quad &\sum_{uvw\in \mathcal{T}}\alpha_{uvw} \\
    \mbox{s.t.} \quad &\sum_{uvw\in \mathcal{T}}\alpha_{uvw}\le \sum_{S\subseteq V,|S|=k}|\{u,v\}\cap S|\cdot \beta_S \quad &\forall u,v\in V\\
    & \sum_{S\subseteq V,|S|=k} \beta_S\le 1 \\
    & \alpha_{uvw}\ge 0 & \forall uvw\in \mathcal{T}\\
    & \beta_S\ge 0 & \forall S\subseteq V,|S|=k.
    \end{aligned}
\end{equation}

For any $u\in V$, set $\gamma_u = \sum_{S\subseteq V,|S|=k}|\{u\}\cap S|\cdot \beta_S$, we have 
\begin{align*}
    \sum_{u\in V}\gamma_u
    &= \sum_{u\in V}\sum_{S\subseteq V,|S|=k}|\{u\}\cap S|\cdot \beta_S\\
    &= k\cdot \sum_{S\subseteq V,|S|=k}\beta_S\\
    &\le k.
\end{align*}

Therefore, ~\ref{lp:badtriangle-dual1} can be rewritten as ~\ref{lp:badtriangle-dual2}.

\begin{equation}\label{lp:badtriangle-dual2}
    \begin{aligned}
    \min_{\alpha,\gamma} \quad &\sum_{uvw\in \mathcal{T}}\alpha_{uvw} \\
    \mbox{s.t.} \quad &\sum_{uvw\in \mathcal{T}}\alpha_{uvw}\le \gamma_u+\gamma_v \quad &\forall u,v\in V\\
    & \sum_{u\in V} \gamma_u\le k \\
    & \gamma_u = \sum_{S\subseteq V,|S|=k}|\{u\}\cap S|\cdot \beta_S & \forall u\in V\\
    & \alpha_{uvw}\ge 0 & \forall uvw\in \mathcal{T}\\
    & \beta_S\ge 0 & \forall S\subseteq V,|S|=k.
    \end{aligned}
\end{equation}


==> not-used/_SymetricCases.tex <==


Assume $|N^+(u)| = \Delta$ for every $u \in V$; we assume $u \in N^+(u)$. In our LP solution, we set $x_{uv} = 1 - \frac{|N^+(u) \cap N^+(v)|}{\Delta}$ for every unordered pair $uv$.  This satisfies the triangle inequalities.

\subsection{The case of top-$n$ norm = $L_1$ norm}
For the top-$n$ norm, which is just the $L_1$ norm, the LP solution is a $2$-approximate. That is, it is at most $2$ times the value of the triangle-packing LP.  For simplicity, here we compare it to the value of the optimal integral solution, i.e, the optimal clustering. 

Below, a bad triangle is a $++-$ triangle. 

For a $+$edge $uv$, its LP cost is 
\begin{align*}
    x_{uv} &= 1 - \frac{|N^+(u) \cap N^+(v)|}{\Delta} = \frac{1}{2}\left(\frac{|N^+(u) \setminus N^+(v)| + |N^+(v) \setminus N^+(u)|}{\Delta}\right) \\
    &= \frac{1}{2\Delta} \cdot \#(\text{bad triangles containing $u$ and $v$}).
\end{align*}
For a $-$edge $uv$, its LP cost is 
\begin{align*}
    1 - x_{uv} &= \frac{|N^+(u) \cap N^+(v)|}{\Delta} = \frac{1}{\Delta} \cdot \#(\text{bad triangles containing $u$ and $v$}).
\end{align*}
So, the value of the LP solution is 
\begin{align*}
    &\quad 2\sum_{uv \in E^+} x_{uv} + 2\sum_{uv \in E^-} (1-x_{uv})\\
    &= \frac{2}{\Delta}\left(\frac{1}{2}\sum_{uv \in E^+}\#(\text{bad triangles containing $u$ and $v$}) + \sum_{uv \in E^-} \#(\text{bad triangles containing $u$ and $v$})\right)\\
    &= \frac{2}{\Delta} \sum_{\text{bad triangles } uvw} \left(\frac12 + \frac12 + 1\right) = \frac{4}{\Delta} \cdot \#(\text{bad triangles}).
\end{align*}

To bound the value of the optimum clustering, we use the following argument. To fix a bad triangle, we need to flip the sign of at least one edge on the triangle. But flipping one edge can fix at most $\Delta$ triangles.  Also, notice that the cost of the solution is twice the number of edges we flipped. So, the optimum value is at least 
\begin{align*}
    \frac{2}{\Delta} \cdot \#(\text{bad triangles}).
\end{align*}

So, the value of the LP solution is at most 2 times the value of the optimum clustering. 

\subsection{The top-$k$ norm case for general $k$}

For now I am not trying to optimize the constant. So, I will just use $O(1)$ everywhere.

Focus on the set $S$ of $k$ vertices with the largest disagreement values w.r.t the LP solution.  For simplicity, let $\calT$ be the set of bad triangles with at least one vertex in $S$. 

Then, the value of the LP solution is at most 
\begin{align*}
    \frac{O(1) \cdot |\calT|}{\Delta}.
\end{align*}

Now consider how the triangles $\calT$ are fixed in the optimum clustering. If a triangle $uvw \in \calT$ has $|\{u, v, w\} \cap S| \geq 2$, then fixing such a triangle will need us to flip one edge incident to $S$. Also, flipping one edge can fix at most $\Delta$ bad triangles. So, this type of bad triangles can be handled. 

So, we consider the case where $|\{u, v, w\} \cap S| = 1$, and the triangle is fixed by flipping the edge not incident to $S$. But it is easy to see that at most $\Delta k$ bad triangles can be fixed this way. If $|\calT| \geq 2\Delta k$, then the number can be ignored. Otherwise, we can consider the $k$ edges not incident to $S$ that fix the most number of bad triangles. For every such an edge, we arbitrarily choose 1 end vertex. Then the $k$ vertices will incur a large cost in the optimum clustering. 

\subsection{Another proof of the top-$k$ norm case for general $k$}
There is another proof of the top-$k$ norm case for general $k$.

For all the $+$edges incident to any $u\in V$, the LP cost is
\begin{align*}
    \quad S^+ &= \sum_{v\in N^+(u) \cap C(u)} \frac{\Delta - |N^+(u) \cap N^+(v)|}{\Delta} + \sum_{v\in N^+(u) \cap \overline{C(u)}} d_{uv}\\
    &\le \frac{1}{2\Delta} \cdot \sum_{v\in N^+(u) \cap C(u)} (|N^+(u) \cap N^-(v)| + |N^-(u) \cap N^+(v)|) + \sum_{v\in N^+(u) \cap \overline{C(u)}} 1\\
    &\le \frac{1}{2\Delta} \cdot \sum_{v\in N^+(u) \cap C(u)} (y(u)+y(v)) + y(u)\\
    &\le \frac{3}{2} \cdot y(u) + \frac{1}{2\Delta} \cdot \sum_{v\in N^+(u)} y(v).
\end{align*}

Define for each $w\in N^+(u)$, $V(w):=\{v\in V|v\in N^-(u)\cap N^+(w)\cap \overline{C(u)}\}$.

For all the $-$edges incident to any $u\in V$, the LP cost is
\begin{align*}
    \quad S^- &= \sum_{v\in N^-(u) \cap \overline{C(u)}} \frac{|N^+(u) \cap N^+(v)|}{\Delta} + \sum_{v\in N^-(u) \cap C(u)} (1-d_{uv})\\
    &\le \sum_{v\in N^-(u) \cap \overline{C(u)}} \frac{|N^+(u) \cap N^+(v)|}{\Delta} + \sum_{v\in N^-(u) \cap C(u)} 1\\
    &\le \sum_{w\in N^+(u) \setminus u} \sum_{v\in V(w)} \frac{1}{\Delta} + y(u)\\
    &= \frac{1}{\Delta} \cdot \sum_{w\in N^+(u) \setminus u, w\in C(u)} |V(w)| + \frac{1}{\Delta} \cdot \sum_{w\in N^+(u), w\in \overline{C(u)}} |V(w)| + y(u)\\
    &\le \frac{1}{\Delta} \cdot \sum_{w\in N^+(u) \setminus u, w\in C(u)} y(w) + \frac{1}{\Delta} \cdot \sum_{w\in N^+(u), w\in \overline{C(u)}} \Delta + y(u)\\
    &\le \frac{1}{\Delta} \cdot \sum_{w\in N^+(u)} y(w) + 2y(u)\\
\end{align*}

Therefore, for any $u\in V$, $\sum_{v\in V} \widehat{d}_{uv}\le \frac{7}{2}\cdot y(u)+\frac{3}{2\Delta}\cdot \sum_{v\in N_u^+}y(v)$.

We arbitrarily choose $k$ \textbf{different} vertices $u_1,u_2,u_3,...,u_k\in V$. Then we have $\sum_{i=1}^k \sum_{v\in N^+(u_i)} y(v)\le \Delta \cdot \mathbf{OPT}_{top-k}$ (Since for all $v\in V$, $y(v)$ can be counted at most $\Delta$ times).

So we have
\begin{align*}
\sum_{i=1}^k \sum_{v\in V} \widehat{d}_{u_iv}&\le \sum_{i=1}^k (\frac{7}{2}y(u_i)+\frac{3}{2\Delta}\sum_{v\in N_{u_i}^+}y(v))\\&\le \frac{7}{2}\sum_{v\in topk}y(v) + \frac{3}{2\Delta}\cdot \sum_{i=1}^k \sum_{v\in N_{u_i}^+}y(v)\\&\le \frac{7}{2}\sum_{v\in topk}y(v) + \frac{3}{2\Delta}\cdot \Delta\sum_{v\in topk}y(v)\\&\le 5\cdot \mathbf{OPT}_{top-k}
\end{align*}


\subsection{Extend: All vertices have similar degrees}

In this subsection we discuss two settings: $x_{uv} = d_{uv} = 1 - \frac{|N^+(u) \cap N^+(v)|}{|N^+(u) \cup N^+(v)|}$ ("correlation metric" setting from DMN23) and $x_{uv} = \widetilde{d}_{uv} = 1 - \frac{|N^+(u) \cap N^+(v)|}{\max \{\Delta_u,\Delta_v\}}$ (our setting).

For a graph where all vertices have similar $+$ degrees, we formally define that for any $u\in V$, $\frac{1}{\sigma}\cdot \Delta \le \Delta_u \le \Delta$. It implies that for any $u,v\in V$, we have $\frac{1}{\sigma}\cdot \Delta_v \le \Delta_u \le \sigma \cdot \Delta_v$.

When set $x_{uv} = d_{uv} = 1 - \frac{|N^+(u) \cap N^+(v)|}{|N^+(u) \cup N^+(v)|}$, we try to analyze the LP cost as follows.

For all the $+$edges incident to any $u\in V$, the LP cost is
\begin{align*}
    \quad S^+ &= \sum_{v\in N^+(u) \cap C(u)} \frac{|N^+(u) \cap N^-(v)| + |N^-(u) \cap N^+(v)|}{|N^+(u) \cup N^+(v)|} + \sum_{v\in N^+(u) \cap \overline{C(u)}} d_{uv}\\
    &\le \frac{1}{\Delta_u} \cdot \sum_{v\in N^+(u) \cap C(u)} (|N^+(u) \cap N^-(v)| + |N^-(u) \cap N^+(v)|) + \sum_{v\in N^+(u) \cap \overline{C(u)}} 1\\
    &\le \frac{1}{\Delta_u} \cdot \sum_{v\in N^+(u) \cap C(u)} (y(u)+y(v)) + y(u)\\
    &\le 2 \cdot y(u) + \frac{1}{\Delta_u} \cdot \sum_{v\in N^+(u)} y(v).
\end{align*}

Define for each $w\in N^+(u)$, $V(w):=\{v\in V|v\in N^-(u)\cap N^+(w)\cap \overline{C(u)}\}$.

For all the $-$edges incident to any $u\in V$, the LP cost is
\begin{align*}
    \quad S^- &= \sum_{v\in N^-(u) \cap \overline{C(u)}} \frac{|N^+(u) \cap N^+(v)|}{|N^+(u) \cup N^+(v)|} + \sum_{v\in N^-(u) \cap C(u)} (1-d_{uv})\\
    &\le \sum_{v\in N^-(u) \cap \overline{C(u)}} \frac{|N^+(u) \cap N^+(v)|}{\Delta_u} + \sum_{v\in N^-(u) \cap C(u)} 1\\
    &\le \sum_{w\in N^+(u) \setminus u} \sum_{v\in V(w)} \frac{1}{\Delta_u} + y(u)\\
    &= \frac{1}{\Delta_u} \cdot \sum_{w\in N^+(u) \setminus u, w\in C(u)} |V(w)| + \frac{1}{\Delta_u} \cdot \sum_{w\in N^+(u), w\in \overline{C(u)}} |V(w)| + y(u)\\
    &\le \frac{1}{\Delta_u} \cdot \sum_{w\in N^+(u) \setminus u, w\in C(u)} y(w) + \frac{1}{\Delta_u} \cdot \sum_{w\in N^+(u), w\in \overline{C(u)}} \Delta_w + y(u)\\
    &\le \frac{1}{\Delta_u} \cdot \sum_{w\in N^+(u) \setminus u, w\in C(u)} y(w) + \frac{1}{\Delta_u} \cdot \sum_{w\in N^+(u), w\in \overline{C(u)}} \sigma \cdot \Delta_u + y(u)\\
    &\le \frac{1}{\Delta_u} \cdot \sum_{w\in N^+(u)} y(w) + (1+\sigma) \cdot y(u)\\
\end{align*}

Therefore, for any $u\in V$, $\sum_{v\in V} \widehat{d}_{uv}\le (3+\sigma)\cdot y(u)+\frac{2}{\Delta_u}\cdot \sum_{v\in N_u^+}y(v)$.

We arbitrarily choose $k$ \textbf{different} vertices $u_1,u_2,u_3,...,u_k\in V$. Then we have $\sum_{i=1}^k \frac{1}{\Delta_{u_i}} \sum_{v\in N^+(u_i)} y(v)\le \frac{\sigma}{\Delta} \cdot \sum_{i=1}^k \sum_{v\in N^+(u_i)} y(v) \le \sigma \cdot \mathbf{OPT}_{top-k}$ (Since for all $v\in V$, $y(v)$ can be counted at most $\Delta$ times).

So we have
\begin{align*}
\sum_{i=1}^k \sum_{v\in V} \widehat{d}_{u_iv}&\le \sum_{i=1}^k ((3+\sigma)\cdot y(u_i)+\frac{2}{\Delta_u}\sum_{v\in N_{u_i}^+}y(v))\\&\le (3+\sigma) \cdot \sum_{v\in topk}y(v) + \frac{2\sigma}{\Delta}\cdot \sum_{i=1}^k \sum_{v\in N_{u_i}^+}y(v)\\&\le (3+\sigma) \cdot \sum_{v\in topk}y(v) + 2\sigma \cdot \sum_{v\in topk}y(v)\\&\le (3+3\sigma)\cdot \mathbf{OPT}_{top-k}
\end{align*}

When set $x_{uv} = \widetilde{d}_{uv} = 1 - \frac{|N^+(u) \cap N^+(v)|}{\max \{\Delta_u,\Delta_v\}}$, our analysis is similar.

For all the $+$edges incident to any $u\in V$, the LP cost is
\begin{align*}
    \quad \widetilde{S}^+ &= \sum_{v\in N^+(u) \cap C(u)} \frac{\max \{\Delta_u,\Delta_v\} - |N^+(u) \cap N^+(v)|}{\max \{\Delta_u,\Delta_v\}} + \sum_{v\in N^+(u) \cap \overline{C(u)}} \widetilde{d}_{uv}\\
    &\le \frac{1}{\Delta_u} \cdot \sum_{v\in N^+(u) \cap C(u)} \max \{|N^+(u) \cap N^-(v)|,|N^-(u) \cap N^+(v)|\} + \sum_{v\in N^+(u) \cap \overline{C(u)}} 1\\
    &\le \frac{1}{\Delta_u} \cdot \sum_{v\in N^+(u) \cap C(u)} (|N^+(u) \cap N^-(v)| + |N^-(u) \cap N^+(v)|) + \sum_{v\in N^+(u) \cap \overline{C(u)}} 1\\
    &\le \frac{1}{\Delta_u} \cdot \sum_{v\in N^+(u) \cap C(u)} (y(u)+y(v)) + y(u)\\
    &\le 2 \cdot y(u) + \frac{1}{\Delta_u} \cdot \sum_{v\in N^+(u)} y(v).
\end{align*}

Define for each $w\in N^+(u)$, $V(w):=\{v\in V|v\in N^-(u)\cap N^+(w)\cap \overline{C(u)}\}$.

For all the $-$edges incident to any $u\in V$, the LP cost is
\begin{align*}
    \quad \widetilde{S}^- &= \sum_{v\in N^-(u) \cap \overline{C(u)}} \frac{|N^+(u) \cap N^+(v)|}{\max \{\Delta_u,\Delta_v\}} + \sum_{v\in N^-(u) \cap C(u)} (1-\widetilde{d}_{uv})\\
    &\le \sum_{v\in N^-(u) \cap \overline{C(u)}} \frac{|N^+(u) \cap N^+(v)|}{\Delta_u} + \sum_{v\in N^-(u) \cap C(u)} 1\\
    &\le \sum_{w\in N^+(u) \setminus u} \sum_{v\in V(w)} \frac{1}{\Delta_u} + y(u)\\
    &= \frac{1}{\Delta_u} \cdot \sum_{w\in N^+(u) \setminus u, w\in C(u)} |V(w)| + \frac{1}{\Delta_u} \cdot \sum_{w\in N^+(u), w\in \overline{C(u)}} |V(w)| + y(u)\\
    &\le \frac{1}{\Delta_u} \cdot \sum_{w\in N^+(u) \setminus u, w\in C(u)} y(w) + \frac{1}{\Delta_u} \cdot \sum_{w\in N^+(u), w\in \overline{C(u)}} \Delta_w + y(u)\\
    &\le \frac{1}{\Delta_u} \cdot \sum_{w\in N^+(u) \setminus u, w\in C(u)} y(w) + \frac{1}{\Delta_u} \cdot \sum_{w\in N^+(u), w\in \overline{C(u)}} \sigma \cdot \Delta_u + y(u)\\
    &\le \frac{1}{\Delta_u} \cdot \sum_{w\in N^+(u)} y(w) + (1+\sigma) \cdot y(u)\\
\end{align*}

We arbitrarily choose $k$ \textbf{different} vertices $u_1,u_2,u_3,...,u_k\in V$. Then we have $\sum_{i=1}^k \sum_{v\in V} \widehat{\widetilde{d}}_{u_iv}\le (3+3\sigma)\cdot \mathbf{OPT}_{top-k}$.

\subsection{Triangle Inequality}
"Fast Combinatorial Algorithms for Min Max Correlation Clustering" already shows that the correlation metric $d_{uv} = 1 - \frac{|N^+(u) \cap N^+(v)|}{|N^+(u) \cup N^+(v)|}$ satisfies the triangle inequality, i.e., for distinct $u,v,w\in V$, $d_{uv}+d_{vw}\ge d_{uw}$.

In this subgraph, we focus on $\widetilde{d}_{uv} = 1 - \frac{|N^+(u) \cap N^+(v)|}{\max \{\Delta_u,\Delta_v\}}$.

\begin{lemma}
    For the $\Delta$-symmetric case, $\widetilde{d}$ satisfies the triangle inequality.
\end{lemma}
\begin{proof}
    For the $\Delta$-symmetric case
    \begin{align*}
        \widetilde{d}_{uv}+\widetilde{d}_{vw}&=1-\frac{|N^+(u)\cap N^+(v)|}{\Delta}+1-\frac{|N^+(v)\cap N^+(w)|}{\Delta}\\
        &=1-\frac{|N^+(u)\cap N^+(v)|+|N^+(v)\cap N^+(w)|-|N^+(v)|}{\Delta}\\
        &\ge 1-\frac{|N^+(u)\cap N^+(v)|+|N^+(v)\cap N^+(w)|-|N^+(v)\cap (N^+(u)\cup N^+(w))|}{\Delta}\\
        &= 1-\frac{|N^+(u)\cap N^+(v)\cap N^+(w)|}{\Delta}\\
        &\ge 1-\frac{|N^+(u)\cap N^+(w)|}{\Delta}\\
        &= \widetilde{d}_{uw}
    \end{align*}
\end{proof}

\begin{lemma}
    For the general case, $\widetilde{d}$ satisfies the triangle inequality.
\end{lemma}
\begin{proof}
    Firstly, we will simply denote the sets $N^+(u),N^+(v),N^+(w)$ as sets $A,B,C$. Then, what we need to prove is $\frac{|A\cap B|}{\max \{|A|,|B|\}}+\frac{|B\cap C|}{\max \{|B|,|C|\}}-\frac{|A\cap C|}{\max \{|A|,|C|\}}\le 1$(let the left-hand side of the inequality be $LHS$). Without loss of generality, let us we assume that $|A|\ge |C|$.

    For shorthand, let the subscripts of the variable $a$ denote the intersections of the three sets(or their complementary sets), e.g., $a_{001}=|\overline{A}\cap \overline{B}\cap C|,a_{010}=|\overline{A}\cap B\cap \overline{C}|,a_{011}=|\overline{A}\cap B\cap C|,a_{100}=|A\cap \overline{B}\cap \overline{C}|$, etc.
    
    When $|A|\ge |C|\ge |B|$, we have
    \small\begin{align*}
        LHS &=\frac{|A\cap B|}{|A|}+\frac{|B\cap C|}{|C|}-\frac{|A\cap C|}{|A|}\\
        &= \frac{|C||A\cap B|+|A||B\cap C|-|C||A\cap C|}{|A||C|}\\
        &= \frac{(a_{001}+a_{011}+a_{101}+a_{111})(a_{110}+a_{111})+(a_{100}+a_{101}+a_{110}+a_{111})(a_{011}+a_{111})-(a_{001}+a_{011}+a_{101}+a_{111})(a_{101}+a_{111})}{(a_{100}+a_{101}+a_{110}+a_{111})(a_{001}+a_{011}+a_{101}+a_{111})}\\
        &=\frac{(a_{001}+a_{011}+a_{101}+a_{111})(a_{110})+(a_{100}+a_{110}+a_{111})(a_{011}+a_{111})-(a_{001}+a_{101})(a_{101})}{(a_{100}+a_{101}+a_{110}+a_{111})(a_{001}+a_{011}+a_{101}+a_{111})}\\
        &\le \frac{(a_{001}+a_{011}+a_{101}+a_{111})(a_{110})+(a_{100}+a_{110}+a_{111})(a_{011}+a_{111})}{(a_{100}+a_{101}+a_{110}+a_{111})(a_{001}+a_{011}+a_{101}+a_{111})}\\
        &= \frac{(a_{001}+a_{011}+a_{101}+a_{111})(a_{110})+(a_{100}+a_{111})(a_{011}+a_{111})+a_{110}(a_{011}+a_{111})}{(a_{001}+a_{011}+a_{101}+a_{111})(a_{110})+(a_{100}+a_{111})(a_{011}+a_{111})+(a_{100}+a_{111})(a_{001}+a_{101})+a_{101}(a_{001}+a_{011}+a_{101}+a_{111})}\\
        &\le \frac{(a_{001}+a_{011}+a_{101}+a_{111})(a_{110})+(a_{100}+a_{111})(a_{011}+a_{111})+(a_{001}+a_{101})(a_{011}+a_{111})}{(a_{001}+a_{011}+a_{101}+a_{111})(a_{110})+(a_{100}+a_{111})(a_{011}+a_{111})+(a_{100}+a_{111})(a_{001}+a_{101})+a_{101}(a_{001}+a_{011}+a_{101}+a_{111})}\\
        &(\because |C|\ge|B|,\quad  \therefore a_{110}+a_{010}+a_{011}+a_{111}\le a_{001}+a_{011}+a_{101}+a_{111},\quad \therefore  a_{110}\le a_{001}+a_{101})\\
        &\le \frac{(a_{001}+a_{011}+a_{101}+a_{111})(a_{110})+(a_{100}+a_{111})(a_{011}+a_{111})+a_{101}(a_{011}+a_{111})+a_{001}(a_{011}+a_{111})}{(a_{001}+a_{011}+a_{101}+a_{111})(a_{110})+(a_{100}+a_{111})(a_{011}+a_{111})+a_{101}(a_{011}+a_{111})+a_{001}(a_{100}+a_{101}+a_{111})}\\
        &\le \frac{(a_{001}+a_{011}+a_{101}+a_{111})(a_{110})+(a_{100}+a_{111})(a_{011}+a_{111})+a_{101}(a_{011}+a_{111})+a_{001}(a_{100}+a_{101}+a_{111})}{(a_{001}+a_{011}+a_{101}+a_{111})(a_{110})+(a_{100}+a_{111})(a_{011}+a_{111})+a_{101}(a_{011}+a_{111})+a_{001}(a_{100}+a_{101}+a_{111})}\\
        &(\because |A|\ge|B|,\quad  \therefore a_{110}+a_{010}+a_{011}+a_{111}\le a_{100}+a_{101}+a_{110}+a_{111},\quad \therefore  a_{011}+a_{111}\le a_{100}+a_{101}+a_{111})\\
        &=1
    \end{align*}

    When $|A|\ge |B|\ge |C|$, we have
    \small\begin{align*}
        LHS &=\frac{|A\cap B|}{|A|}+\frac{|B\cap C|}{|B|}-\frac{|A\cap C|}{|A|}\\
        &= \frac{|B||A\cap B|+|A||B\cap C|-|B||A\cap C|}{|A||B|}\\
        &= \frac{(a_{010}+a_{011}+a_{110}+a_{111})(a_{110}+a_{111})+(a_{100}+a_{101}+a_{110}+a_{111})(a_{011}+a_{111})-(a_{010}+a_{011}+a_{110}+a_{111})(a_{101}+a_{111})}{(a_{100}+a_{101}+a_{110}+a_{111})(a_{010}+a_{011}+a_{110}+a_{111})}\\
        &=\frac{a_{110}(a_{010}+a_{011}+a_{110}+a_{111})+(a_{100}+a_{111})(a_{011}+a_{111})+a_{110}(a_{011}+a_{111})-a_{101}(a_{010}+a_{110})}{a_{110}(a_{010}+a_{011}+a_{110}+a_{111})+(a_{100}+a_{111})(a_{011}+a_{111})+(a_{100}+a_{111})(a_{010}+a_{110})+a_{101}(a_{010}+a_{011}+a_{110}+a_{111})}\\
        &\le \frac{a_{110}(a_{010}+a_{011}+a_{110}+a_{111})+(a_{100}+a_{111})(a_{011}+a_{111})+a_{110}(a_{011}+a_{111})}{a_{110}(a_{010}+a_{011}+a_{110}+a_{111})+(a_{100}+a_{111})(a_{011}+a_{111})+a_{110}(a_{100}+a_{101}+a_{111})}\\
        &\le \frac{a_{110}(a_{010}+a_{011}+a_{110}+a_{111})+(a_{100}+a_{111})(a_{011}+a_{111})+a_{110}(a_{100}+a_{101}+a_{111})}{a_{110}(a_{010}+a_{011}+a_{110}+a_{111})+(a_{100}+a_{111})(a_{011}+a_{111})+a_{110}(a_{100}+a_{101}+a_{111})}\\
        &(\because |A|\ge|B|,\quad  \therefore a_{110}+a_{010}+a_{011}+a_{111}\le a_{100}+a_{101}+a_{110}+a_{111},\quad \therefore  a_{011}+a_{111}\le a_{100}+a_{101}+a_{111})\\
        &=1
    \end{align*}

    When $|B|\ge |A|\ge |C|$, we have
    \small\begin{align*}
        LHS &=\frac{|A\cap B|}{|B|}+\frac{|B\cap C|}{|B|}-\frac{|A\cap C|}{|A|}\\
        &= \frac{|A||A\cap B|+|A||B\cap C|-|B||A\cap C|}{|A||B|}\\
       &= \frac{(a_{100}+a_{101}+a_{110}+a_{111})(a_{110}+a_{111})+(a_{100}+a_{101}+a_{110}+a_{111})(a_{011}+a_{111})-(a_{010}+a_{011}+a_{110}+a_{111})(a_{101}+a_{111})}{(a_{100}+a_{101}+a_{110}+a_{111})(a_{010}+a_{011}+a_{110}+a_{111})}\\
        &=\frac{(a_{100}+a_{101}+a_{110}+a_{111})(a_{110}+a_{111})+(a_{100}+a_{101}+a_{110}+a_{111})(a_{011}+a_{111})-(a_{010}+a_{011}+a_{110}+a_{111})(a_{101}+a_{111})}{(a_{100}+a_{101}+a_{110}+a_{111})(a_{010}+a_{011}+a_{110}+a_{111})}\\
        &=\frac{2a_{111}(a_{100}+a_{101}+a_{110}+a_{111})+(a_{100}+a_{110})(a_{110}+a_{011})-(a_{010}+a_{111})(a_{101}+a_{111})}{a_{111}(a_{100}+a_{101}+a_{110}+a_{111})+(a_{010}+a_{011}+a_{110})(a_{100}+a_{101}+a_{110}+a_{111})}\\
        &\le \frac{2a_{111}(a_{100}+a_{101}+a_{110}+a_{111})+(a_{100}+a_{110})(a_{110}+a_{011})-a_{111}(a_{101}+a_{111})}{a_{111}(a_{100}+a_{101}+a_{110}+a_{111})+(a_{100}+a_{110})(a_{110}+a_{011})+a_{111}(a_{010}+a_{011}+a_{110})}\\
        &= \frac{a_{111}(a_{100}+a_{101}+a_{110}+a_{111})+(a_{100}+a_{110})(a_{110}+a_{011})+a_{111}(a_{100}+a_{110})}{a_{111}(a_{100}+a_{101}+a_{110}+a_{111})+(a_{100}+a_{110})(a_{110}+a_{011})+a_{111}(a_{010}+a_{011}+a_{110})}\\
        &\le \frac{a_{111}(a_{100}+a_{101}+a_{110}+a_{111})+(a_{100}+a_{110})(a_{110}+a_{011})+a_{111}(a_{010}+a_{011}+a_{110})}{a_{111}(a_{100}+a_{101}+a_{110}+a_{111})+(a_{100}+a_{110})(a_{110}+a_{011})+a_{111}(a_{010}+a_{011}+a_{110})}\\
        &(\because |A|\le|B|,\quad  \therefore a_{100}+a_{101}+a_{110}+a_{111}\le a_{110}+a_{010}+a_{011}+a_{111},\quad \therefore  a_{100}\le a_{010}+a_{011})\\
        &=1
    \end{align*}

    So we have proved that $\frac{|A\cap B|}{\max \{A,B\}}+\frac{|B\cap C|}{\max \{B,C\}}-\frac{|A\cap C|}{\max \{A,C\}}\le 1$.
\end{proof}

Note that "Fast Combinatorial Algorithms for Min Max Correlation Clustering" already proved that if $g$ is a $\delta$-semi-metric on the set $V$, instead of a true semi-metric (i.e., $1$-semi-metric), then the KMZ algorithm loses a factor of $1 + \delta + \delta^2 + \delta^3 + \delta^4$.

==> not-used/_removed.tex <==
{\color{gray}\begin{align*}
    x_{uv} + x_{uw} &\geq x_{vw} \\
\Leftrightarrow 1-\frac{|N_{H}(u)\cap N_{H}(v)|}{\mathrm{\max}(d(u), d(v))} &+ 1-\frac{|N_{H}(u)\cap N_{H}(w)|}{\mathrm{\max}(d(u), d(w))} \geq 1-\frac{|N_{H}(v)\cap N_{H}(w)|}{\mathrm{\max}(d(v), d(w))} \\
\Leftrightarrow 1 + \frac{|N_{H}(v)\cap N_{H}(w)|}{\mathrm{\max}(d(v), d(w))} &\geq \frac{|N_{H}(u)\cap N_{H}(v)|}{\mathrm{\max}(d(u), d(v))} + \frac{|N_{H}(u)\cap N_{H}(w)|}{\mathrm{\max}(d(u), d(w))} \\
\Leftrightarrow 1 + \frac{|N_{H}(v)\cap N_{H}(w)|}{d(v)} &\geq \frac{|N_{H}(u)\cap N_{H}(v)|}{\mathrm{\max}(d(u), d(v))} + \frac{|N_{H}(u)\cap N_{H}(w)|}{\mathrm{\max}(d(u), d(w))} \\
\Leftarrow 1 + \frac{|N_{H}(v)\cap N_{H}(w)|}{\mathrm{\max}(d(u), d(v))} &\geq \frac{|N_{H}(u)\cap N_{H}(v)|}{\mathrm{\max}(d(u), d(v))} + \frac{|N_{H}(u)\cap N_{H}(w)|}{\mathrm{\max}(d(u), d(w))} \\ 
\Leftrightarrow 1 - \frac{|N_{H}(u)\cap N_{H}(w)|}{\mathrm{\max}(d(u), d(w))} &\geq \frac{|N_{H}(u)\cap N_{H}(v)|}{\mathrm{\max}(d(u), d(v))} - \frac{|N_{H}(v)\cap N_{H}(w)|}{\mathrm{\max}(d(u), d(v))}
\end{align*}

The left side is no less than 0, when $|N_{H}(u)\cap N_{H}(v)| \leq |N_{H}(v)\cap N_{H}(w)|$, the right side is greater or equal to $0$ and the above inequality holds automatically. Therefore, we assume $|N_{H}(u)\cap N_{H}(v)| > |N_{H}(v)\cap N_{H}(w)|$. Note that we have 
\begin{align*}
   N_{H}(u)\cap N_{H}(v) \setminus \big( N_{H}(v)\cap N_{H}(w) \big) \subset N_H(u) \setminus N_H(w)
\end{align*}
which implies
\begin{align*}
    \mathrm{\max}(d(u), d(w)) - |N_{H}(u)\cap N_{H}(w)| &\geq d(u) - |N_{H}(u)\cap N_{H}(w)| \\ 
    &\geq |N_{H}(u)\cap N_{H}(v)| - |N_{H}(v)\cap N_{H}(w)|
\end{align*}
 then we have 
 \begin{align*}
     1 - \frac{|N_{H}(u)\cap N_{H}(w)|}{\mathrm{\max}(d(u), d(w))} &\geq \frac{|N_{H}(u)\cap N_{H}(v)| - |N_{H}(v)\cap N_{H}(w)|}{\mathrm{\max}(d(u), d(w))} \\
     &\geq \frac{|N_{H}(u)\cap N_{H}(v)| - |N_{H}(v)\cap N_{H}(w)|}{\mathrm{\max}(d(u), d(v))}
 \end{align*}
     which gives us the inequality.}




%Let $ $ be the set of negative edges that are in same clustering of $\mathcal{C}$, $ $ be the set of negative edges that are in different clustering of $\mathcal{C}$ and it has at least one common neighborhood in graph $H$.%respectively be the sets of edges incident to $u$ that are in $E \setminus E_H$ %that are deleted at step \ref{alg:pre-clusteringlpfirst} in Algorithm~\ref{alg:pre-clusteringlp} and are 
%and not cut in $\mathcal{C}$, cut in $\mathcal{C}$, and in $H$ and not cut in $\mathcal{C}$. 
%Then we can bound $\sum_{u \in U} y^{+}(u)$ using $\varphi_1$, $\varphi_3$ and $\varphi_4$. Recall that we already have the bound for $\varphi_1$ by lemma \ref{lem:deletededgesatstep1}. 
% We first bound $y^+(u)$ for every $u \in U$. Notice that
% \begin{align*}
%     y^{+}(u) &= \cost^1_x(u) + \cost^3_x(u) + \cost^4_x(u) % \sum_{uv \in \varphi_1(u)} x_{uv} + \sum_{uv \in \varphi_3(u)} x_{uv} + \sum_{uv \in \varphi_4(u)} x_{uv}\\
%     \leq |\varphi_1(u)| + \cost^{+}_{\mathcal{C}}(u) +  \cost^4_x(u).
% \end{align*}




{\color{gray}
On the other hand, we can rewrite the $f_3(u)$ as  
\begin{align*}
&\sum_{\substack{u \in U, uv \in \varphi_4(u)\\(u,w) \in \varphi_1(u)}} \frac{\cost_{\mathcal{C}}(u) + \cost_{\mathcal{C}}(w)}{\beta \cdot M_{uv}M_{uw}} + \sum_{\substack{u \in U, uv \in \varphi_4(u)\\(v,w) \in \varphi_1(v)}} \frac{\cost_{\mathcal{C}}(v) + \cost_{\mathcal{C}}(w)}{\beta \cdot M_{uv}M_{vw}} \\
     &+ \sum_{u \in U, uv \in \varphi_4(u)} \frac{\cost_{\mathcal{C}}(u)+ \cost_{\mathcal{C}}(v)}{M_{uv}}+ \sum_{u \in U, uv \in \varphi_1(u)} \frac{\cost_{\mathcal{C}}(u)+ \cost_{\mathcal{C}}(v)}{\beta\cdot M_{uv}} \\
&= \sum_{\substack{u \in U, uv \in \varphi_4(u)\\(u,w) \in \varphi_1(u)}} \frac{\cost_{\mathcal{C}}(u)}{\beta \cdot M_{uv}M_{uw}} + \sum_{\substack{u \in U, uv \in \varphi_4(u)\\(u,w) \in \varphi_1(u)}} \frac{\cost_{\mathcal{C}}(w)}{\beta \cdot M_{uv}M_{uw}} + \sum_{\substack{u \in U, uv \in \varphi_4(u)\\(v,w) \in \varphi_1(v)}} \frac{\cost_{\mathcal{C}}(v)}{\beta \cdot M_{uv}M_{vw}} \\
     &+ \sum_{\substack{u \in U, uv \in \varphi_4(u)\\(v,w) \in \varphi_1(v)}} \frac{\cost_{\mathcal{C}}(w)}{\beta \cdot M_{uv}M_{vw}} + \sum_{u \in U, uv \in \varphi_4(u)} \frac{\cost_{\mathcal{C}}(u)}{M_{uv}}+ \sum_{u \in U, uv \in \varphi_4(u)} \frac{\cost_{\mathcal{C}}(v)}{M_{uv}} \\
     &+  \sum_{u \in U, uv \in \varphi_1(u)} \frac{\cost_{\mathcal{C}}(u)}{\beta\cdot M_{uv}} + \sum_{u \in U, uv \in \varphi_1(u)} \frac{\cost_{\mathcal{C}}(v)}{\beta\cdot M_{uv}} \\
     &= \sum_{\substack{u \in U, uv \in \varphi_4(u)\\(u,w) \in \varphi_1(u)}} \frac{\cost_{\mathcal{C}}(u)}{\beta \cdot M_{uv}M_{uw}} + \sum_{\substack{u \in V, w \in U, (w,u) \in \varphi_1(w)\\(w,v) \in \varphi_4(w)}} \frac{\cost_{\mathcal{C}}(u)}{\beta \cdot M(w, u)M(w, v)} + \sum_{\substack{u \in V, w \in U, (w, u) \in \varphi_4(w) \\uv \in \varphi_1(u)}} \frac{\cost_{\mathcal{C}}(u)}{\beta \cdot M_{uv}M_{uw}} \\
     &+ \sum_{\substack{u \in V, w \in U, (w,v) \in \varphi_4(w)\\(v,u) \in \varphi_1(v)}} \frac{\cost_{\mathcal{C}}(u)}{\beta \cdot M_{uv}M_{vw}} + \sum_{u \in U, uv \in \varphi_4(u)} \frac{\cost_{\mathcal{C}}(u)}{M_{uv}}+ \sum_{u \in V, v \in U, (v,u) \in \varphi_4(v)} \frac{\cost_{\mathcal{C}}(u)}{M_{uv}} \\
     &+  \sum_{u \in U, uv \in \varphi_1(u)} \frac{\cost_{\mathcal{C}}(u)}{\beta\cdot M_{uv}} + \sum_{u \in V, v \in U, (v,u) \in \varphi_1(v)} \frac{\cost_{\mathcal{C}}(u)}{\beta\cdot M_{uv}} \\
% &\leq \sum_{\substack{u \in V, d(u) \geq d(v), \\ uv \in \varphi_4(u), u \in U}} \frac{|\varphi_1(u)| + |\varphi_3(u)|}{d(u)} + \sum_{\substack{u \in V, d(u) \geq d(v) \\ (v, u) \in \varphi_4(v), v \in U}} \frac{|\varphi_1(u)| + |\varphi_3(u)|}{d(u)}
\end{align*}
For any fixed $u\in V$, the coefficient is at most 
\begin{align*}
&\sum_{\substack{uv \in \varphi_4(u)\\(u,w) \in \varphi_1(u)}} \frac{1}{\beta \cdot M_{uv}M_{uw}} + \sum_{\substack{w \in U, (w,u) \in \varphi_1(w)\\(w,v) \in \varphi_4(w)}} \frac{1}{\beta \cdot M(w, u)M(w, v)} + \sum_{\substack{w \in U, (w, u) \in \varphi_4(w) \\uv \in \varphi_1(u)}} \frac{1}{\beta \cdot M_{uv}M_{uw}} \\
     &+ \sum_{\substack{w \in U, (w,v) \in \varphi_4(w)\\(v,u) \in \varphi_1(v)}} \frac{1}{\beta \cdot M_{uv}M_{vw}} + \sum_{ uv \in \varphi_4(u)} \frac{1}{M_{uv}}+ \sum_{v \in U, (v,u) \in \varphi_4(v)} \frac{1}{M_{uv}} \\
     &+  \sum_{uv \in \varphi_1(u)} \frac{1}{\beta\cdot M_{uv}} + \sum_{v \in U, (v,u) \in \varphi_1(v)} \frac{1}{\beta\cdot M_{uv}} \\ 
     &\leq  \frac{|\varphi_1(u)|\cdot|\varphi_4(u)|}{\beta \cdot d(u) \cdot d(u)} + \frac{|\varphi_1(u)|}{\beta \cdot d(u)} + \frac{|\varphi_1(u)|\cdot|\varphi_4(u)|}{\beta \cdot d(u) \cdot d(u)} +\frac{|\varphi_1(u)|}{\beta \cdot d(u)} +  \frac{|\varphi_4(u)|}{d(u)}+ \frac{|\varphi_4(u)|}{d(u)} 
     +  \frac{|\varphi_1(u)|}{\beta\cdot d(u)} + \frac{|\varphi_1(u)|}{\beta\cdot d(u)} \\
     &\leq \frac{1}{\beta} \cdot \frac{2|\varphi_1(u)|\cdot|\varphi_4(u)| + 4|\varphi_1(u)| \cdot d(u) + 2\beta |\varphi_4(u)| \cdot d(u)}{d(u) \cdot d(u)} \\
     &\leq \frac{1}{\beta} \cdot \frac{2d(u)\cdot|\varphi_4(u)| + 4|\varphi_1(u)| \cdot d(u) + 2 |\varphi_4(u)| \cdot d(u)}{d(u) \cdot d(u)} \\
     &\leq \frac{1}{\beta} \cdot \frac{4(|\varphi_1(u)|+|\varphi_4(u)|)\cdot d(u)}{d(u) \cdot d(u)} \leq \frac{4}{\beta}
\end{align*}
Therefore, for any $\beta \leq 0.6$, we can bound $f_3(u)$ by
\begin{align*}
    f_3(u) \leq \mathrm{\max}(\frac{4}{\beta}, \frac{2.5}{\beta} + 2)) \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'} \cost_{\mathcal{C}}(w) \leq \frac{4}{\beta} \cdot \cost^k_G(\mathcal{C})
\end{align*}
and we can bound $\sum_{u \in U} y^{+}(u)$ by
\begin{align*}
    \sum_{u \in U} y^{+}(u) 
    &\leq \sum_{u \in U} |\varphi_1(u)| + \sum_{u \in U} \cost^{+}_{\mathcal{C}}(u) + \sum_{u \in U, uv \in \varphi_4(u)} x_{uv} \\
    &\leq f_3(u) + \sum_{u \in U} \cost^{+}_{\mathcal{C}}(u) \leq (1 + \frac{4}{\beta}) \cdot \cost^k_G(\mathcal{C})
\end{align*}
}





% The sum of the coefficients is at most
% \begin{align*}
% \sum_{u \in V} c(u) &\leq \sum_{\substack{u \in U, uv \in \varphi_4(u)\\(u,w) \in \varphi_1(u)}} \frac{2}{\beta \cdot M_{uv}M_{uw}} + \sum_{\substack{u \in U, uv \in \varphi_4(u)\\(v,w) \in \varphi_1(v)}} \frac{2}{\beta \cdot M_{uv}M_{vw}} \\ 
% & \quad + \sum_{u \in U, uv \in \varphi_4(u)} \frac{2}{M_{uv}} + \sum_{u \in U, uv \in \varphi_1(u)} \frac{2}{\beta\cdot M_{uv}}
% \\ 
% &\leq \sum_{u \in U} \big( \frac{2|\varphi_1(u)||\varphi_4(u)|}{\beta \cdot d(u) \cdot d(u)} + \frac{2|\varphi_4(u)|}{\beta \cdot d(u)} 
% + \frac{2|\varphi_4(u)|}{d(u)} + \frac{2|\varphi_1(u)|}{\beta\cdot d(u)} \big)\\
% &\leq \sum_{u \in U} \big( \frac{2|\varphi_1(u)||\varphi_4(u)|}{\beta \cdot (|\varphi_1(u)| + |\varphi_4(u)|)^2 } + \frac{2|\varphi_4(u)| + 2|\varphi_1(u)|}{\beta \cdot d(u)} 
% + \frac{2|\varphi_4(u)|}{d(u)} \big) \\
% &\leq \sum_{u \in U} (\frac{2.5}{\beta} + 2) = k \cdot (\frac{2.5}{\beta} + 2)
% \end{align*}
% On the other hand, we can rewrite the $f_3(u)$ as  
% \begin{align*}
% &\sum_{\substack{u \in U, uv \in \varphi_4(u)\\(u,w) \in \varphi_1(u)}} \frac{\cost_{\mathcal{C}}(u) + \cost_{\mathcal{C}}(w)}{\beta \cdot M_{uv}M_{uw}} + \sum_{\substack{u \in U, uv \in \varphi_4(u)\\(v,w) \in \varphi_1(v)}} \frac{\cost_{\mathcal{C}}(v) + \cost_{\mathcal{C}}(w)}{\beta \cdot M_{uv}M_{vw}} \\
%      &+ \sum_{u \in U, uv \in \varphi_4(u)} \frac{\cost_{\mathcal{C}}(u)+ \cost_{\mathcal{C}}(v)}{M_{uv}}+ \sum_{u \in U, uv \in \varphi_1(u)} \frac{\cost_{\mathcal{C}}(u)+ \cost_{\mathcal{C}}(v)}{\beta\cdot M_{uv}} \\
% &= \sum_{\substack{u \in U, uv \in \varphi_4(u)\\(u,w) \in \varphi_1(u)}} \frac{\cost_{\mathcal{C}}(u)}{\beta \cdot M_{uv}M_{uw}} + \sum_{\substack{u \in U, uv \in \varphi_4(u)\\(u,w) \in \varphi_1(u)}} \frac{\cost_{\mathcal{C}}(w)}{\beta \cdot M_{uv}M_{uw}} + \sum_{\substack{u \in U, uv \in \varphi_4(u)\\(v,w) \in \varphi_1(v)}} \frac{\cost_{\mathcal{C}}(v)}{\beta \cdot M_{uv}M_{vw}} \\
%      &+ \sum_{\substack{u \in U, uv \in \varphi_4(u)\\(v,w) \in \varphi_1(v)}} \frac{\cost_{\mathcal{C}}(w)}{\beta \cdot M_{uv}M_{vw}} + \sum_{u \in U, uv \in \varphi_4(u)} \frac{\cost_{\mathcal{C}}(u)}{M_{uv}}+ \sum_{u \in U, uv \in \varphi_4(u)} \frac{\cost_{\mathcal{C}}(v)}{M_{uv}} \\
%      &+  \sum_{u \in U, uv \in \varphi_1(u)} \frac{\cost_{\mathcal{C}}(u)}{\beta\cdot M_{uv}} + \sum_{u \in U, uv \in \varphi_1(u)} \frac{\cost_{\mathcal{C}}(v)}{\beta\cdot M_{uv}} \\
%      &= \sum_{\substack{u \in U, uv \in \varphi_4(u)\\(u,w) \in \varphi_1(u)}} \frac{\cost_{\mathcal{C}}(u)}{\beta \cdot M_{uv}M_{uw}} + \sum_{\substack{u \in V, w \in U, (w,u) \in \varphi_1(w)\\(w,v) \in \varphi_4(w)}} \frac{\cost_{\mathcal{C}}(u)}{\beta \cdot M(w, u)M(w, v)} + \sum_{\substack{u \in V, w \in U, (w, u) \in \varphi_4(v) \\uv \in \varphi_1(u)}} \frac{\cost_{\mathcal{C}}(u)}{\beta \cdot M_{uv}M_{uw}} \\
%      &+ \sum_{\substack{u \in V, w \in U, (w,v) \in \varphi_4(w)\\(v,u) \in \varphi_1(v)}} \frac{\cost_{\mathcal{C}}(u)}{\beta \cdot M_{uv}M_{vw}} + \sum_{u \in U, uv \in \varphi_4(u)} \frac{\cost_{\mathcal{C}}(u)}{M_{uv}}+ \sum_{u \in V, v \in U, (v,u) \in \varphi_4(v)} \frac{\cost_{\mathcal{C}}(u)}{M_{uv}} \\
%      &+  \sum_{u \in U, uv \in \varphi_1(u)} \frac{\cost_{\mathcal{C}}(u)}{\beta\cdot M_{uv}} + \sum_{u \in V, v \in U, (v,u) \in \varphi_1(v)} \frac{\cost_{\mathcal{C}}(u)}{\beta\cdot M_{uv}} \\
% % &\leq \sum_{\substack{u \in V, d(u) \geq d(v), \\ uv \in \varphi_4(u), u \in U}} \frac{|\varphi_1(u)| + |\varphi_3(u)|}{d(u)} + \sum_{\substack{u \in V, d(u) \geq d(v) \\ (v, u) \in \varphi_4(v), v \in U}} \frac{|\varphi_1(u)| + |\varphi_3(u)|}{d(u)}
% \end{align*}
% For any fixed $u\in V$, the coefficient is at most 
% \begin{align*}
% &\sum_{\substack{uv \in \varphi_4(u)\\(u,w) \in \varphi_1(u)}} \frac{1}{\beta \cdot M_{uv}M_{uw}} + \sum_{\substack{w \in U, (w,u) \in \varphi_1(w)\\(w,v) \in \varphi_4(w)}} \frac{1}{\beta \cdot M(w, u)M(w, v)} + \sum_{\substack{w \in U, (w, u) \in \varphi_4(v) \\uv \in \varphi_1(u)}} \frac{1}{\beta \cdot M_{uv}M_{uw}} \\
%      &+ \sum_{\substack{w \in U, (w,v) \in \varphi_4(w)\\(v,u) \in \varphi_1(v)}} \frac{1}{\beta \cdot M_{uv}M_{vw}} + \sum_{ uv \in \varphi_4(u)} \frac{1}{M_{uv}}+ \sum_{v \in U, (v,u) \in \varphi_4(v)} \frac{1}{M_{uv}} \\
%      &+  \sum_{uv \in \varphi_1(u)} \frac{1}{\beta\cdot M_{uv}} + \sum_{v \in U, (v,u) \in \varphi_1(v)} \frac{1}{\beta\cdot M_{uv}} \\ 
%      &\leq  \frac{|\varphi_1(u)|\cdot|\varphi_4(u)|}{\beta \cdot d(u) \cdot d(u)} + \frac{|\varphi_1(u)|}{\beta \cdot d(u)} + \frac{|\varphi_1(u)|\cdot|\varphi_4(u)|}{\beta \cdot d(u) \cdot d(u)} +\frac{|\varphi_1(u)|}{\beta \cdot d(u)} +  \frac{|\varphi_4(u)|}{d(u)}+ \frac{|\varphi_4(u)|}{d(u)} 
%      +  \frac{|\varphi_1(u)|}{\beta\cdot d(u)} + \frac{|\varphi_1(u)|}{\beta\cdot d(u)} \\
%      &\leq \frac{1}{\beta} \cdot \frac{2|\varphi_1(u)|\cdot|\varphi_4(u)| + 4|\varphi_1(u)| \cdot d(u) + 2\beta |\varphi_4(u)| \cdot d(u)}{d(u) \cdot d(u)} \\
%      &\leq \frac{1}{\beta} \cdot \frac{2d(u)\cdot|\varphi_4(u)| + 4|\varphi_1(u)| \cdot d(u) + 2 |\varphi_4(u)| \cdot d(u)}{d(u) \cdot d(u)} \\
%      &\leq \frac{1}{\beta} \cdot \frac{4(|\varphi_1(u)|+|\varphi_4(u)|)\cdot d(u)}{d(u) \cdot d(u)} \leq \frac{4}{\beta}
% \end{align*}
% Therefore, for any $\beta \leq 0.6$, we can bound $f_3(u)$ by
% \begin{align*}
%     f_3(u) \leq \mathrm{\max}(\frac{4}{\beta}, \frac{2.5}{\beta} + 2)) \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'} \cost_{\mathcal{C}}(w) \leq \frac{4}{\beta} \cdot \cost^k_G(\mathcal{C})
% \end{align*}
% and we can bound $\sum_{u \in U} y^{+}(u)$ by
% \begin{align*}
%     \sum_{u \in U} y^{+}(u) 
%     &\leq \sum_{u \in U} |\varphi_1(u)| + \sum_{u \in U} \cost^{+}_{\mathcal{C}}(u) + \sum_{u \in U, uv \in \varphi_4(u)} x_{uv} \\
%     &\leq f_3(u) + \sum_{u \in U} \cost^{+}_{\mathcal{C}}(u) \leq (1 + \frac{4}{\beta}) \cdot \cost^k_G(\mathcal{C})
% \end{align*}


% Again, the sum of the coefficients is 
% \begin{align*}
%     \sum_{\substack{u \in U, uv \in \varphi_4(u) \\ w = \mathrm{arg\max}_{w\in \{u,v\}} d(w)}} \frac{1}{d(w)} \leq \sum_{\substack{u \in U, uv \in \varphi_4(u) }} \frac{1}{d(u)} \leq \sum_{u \in U} 1 = k
% \end{align*}
% We rewrite the second term as 
% \begin{align*}
%     \sum_{\substack{u \in U, uv \in \varphi_4(u) \\ w = \mathrm{arg\max}_{w\in \{u,v\}} d(w) \\ \Tilde{w} \in \{ u, v\} / \{ w \}}} \frac{|\varphi_1(\Tilde{w})| + \cost^{-}_{\mathcal{C}}}(\Tilde{w})}{d(w)} = \sum_{\substack{u \in V, d(u) \leq d(v), \\ uv \in \varphi_4(u), u \in U \\ or (v, u) \in \varphi_4(v), v \in U}} \frac{|\varphi_1(u)| + \cost^{-}_{\mathcal{C}}}(u)}{d(v)} 
% \end{align*}
% and the coefficient for each $u\in V$ is at most 
% \begin{align*}
%  \sum_{\substack{u \in V, d(u) \leq d(v), \\ uv \in \varphi_4(u), u \in U \\ or (v, u) \in \varphi_4(v), v \in U}} \frac{1}{d(v)} \leq \sum_{\substack{u \in V, d(u) \geq d(v), \\ uv \in \varphi_4(u), u \in U}} \frac{1}{d(v)} + \sum_{\substack{u \in V, d(u) \geq d(v) \\ (v, u) \in \varphi_4(v), v \in U}} \frac{1}{d(v)} = 2
% \end{align*}

% so the second term can be bounded by 
% \begin{align*}
%     &\sum_{\substack{u \in U, uv \in \varphi_4(u) \\ w = \mathrm{arg\max}_{w\in \{u,v\}} d(w) \\ \Tilde{w} \in \{ u, v\} / \{ w \}}} \frac{|\varphi_1(\Tilde{w})| + \cost^{-}_{\mathcal{C}}}(\Tilde{w})}{d(w)} \\ \leq& 2 \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}|\varphi_1(w)| + 2 \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}\cost^{-}_{\mathcal{C}}}(w)
% \end{align*}
% Combining together, we have 
% \begin{align*}
%     &\sum_{u \in U, uv \in \varphi_4(u)} x_{uv} \\
%     &\leq 2 \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}|\varphi_1(w)| + 4\cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}|\varphi_1(w)| + 2\cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}\cost^{-}_{\mathcal{C}}}(w) \\
%     &\leq 2\cost^k_G(\mathcal{C}) + 4 \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}|\varphi_1(w)|
% \end{align*}
% and 
% \begin{align*}
%     \sum_{u \in U} y^{+}(u)
%     &\leq \sum_{u \in U} |\varphi_1(u)| + \sum_{u \in U} |\varphi_3(u)| + \sum_{u \in U, uv \in \varphi_4(u)} x_{uv} \\
%     &\leq 3\cost^k_G(\mathcal{C}) + 5 \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}|\varphi_1(w)| \\
%     &\leq (3 + \frac{10}{\beta}) \cost^k_G(\mathcal{C})
% \end{align*}


% \begin{proof}
% Let $\varphi_1(u) = \{uv \mid uv \in E(G) \setminus E(H), C(u) = C(v) \}$ be the set of edges that are deleted at \ref{alg:pre-clusteringlpfirst} in Algorithm~\ref{alg:pre-clusteringlp} and are not cut in $\mathcal{C}$, $\varphi_3(u) = \{uv \mid uv \in E(G), C(u) \not= C(v) \}$ be the set of edges that are cut in $\mathcal{C}$. $\varphi_4(u) = \{uv \mid uv \in E(H), C(u) = C(v) \} $ be the set of edges that in $H$ and not cut in $\mathcal{C}$. Then we can bound $\sum_{u \in U} y^{+}(u)$ using $\varphi_1$, $\varphi_3$ and $\varphi_4$. Recall that we already have the bound for $\varphi_1$ by lemma \ref{lem:deletededgesatstep1}.
% \begin{align*}
%     \sum_{u \in U} y^{+}(u) &\leq \sum_{u \in U} \big( \sum_{uv \in \varphi_1(u)} x_{uv} + \sum_{uv \in \varphi_3(u)} x_{uv} + \sum_{uv \in \varphi_4(u)} x_{uv} \big) \\
%     &\leq \sum_{u \in U} |\varphi_1(u)| + \sum_{u \in U} |\varphi_3(u)| + \sum_{u \in U, uv \in \varphi_4(u)} x_{uv}
% \end{align*}
% We have to bound $\sum_{u \in U, uv \in \varphi_4(u)} x_{uv}$. Fix node $u$, for any edge $uv \in \varphi_4(u)$, Algorithm \ref{alg:pre-clusteringlp} keep it at the end, so we know that $|N(u) \Delta N(v)| \leq \beta \cdot \max(d(u), d(v))$ and $  (1 - \beta) d(v) \leq d(u)  \leq \frac{d(v)}{1 - \beta}$,
% \begin{align*}
%     x_{uv} &\leq 1 - \frac{|N_{H}(u) \cap N_{H}(v)|}{\mathrm{\max}(d(u), d(v))} \leq \frac{\mathrm{\max}(d(u), d(v)) - |N_{H}(u) \cap N_{H}(v)|}{\mathrm{\max}(d(u), d(v))} 
% \end{align*}
% Therefore, 
% \begin{align*}
%     \sum_{u \in U, uv \in \varphi_4(u)} x_{uv} &\leq \sum_{\substack{u \in U, uv \in \varphi_4(u) \\ w = \mathrm{arg\max}_{w\in \{u,v\}}d(w)}} \frac{|\varphi_1(w)| + |\varphi_3(w)| + |\varphi_4(w)| - |N_H(u) \cap N_H(v)|}{d(w)} \\
%     &\leq \sum_{\substack{u \in U, uv \in \varphi_4(u) \\ w = \mathrm{arg\max}_{w\in \{u,v\}}d(w)}}\frac{|\varphi_1(w)| + |\varphi_3(w)|}{d(w)} + \sum_{\substack{u \in U, uv \in \varphi_4(u) \\ w = \mathrm{arg\max}_{w\in \{u,v\}}d(w)}} \frac{|\varphi_4(w)| - |N_H(u) \cap N_H(v)|}{d(w)}
% \end{align*}
% For the first and second terms, we will use the same strategy to bound the value. We treat each term as a fractional combination of $\varphi_1$ $\varphi_3$ function. If we can show that the coefficient of $\varphi_1(w)$ and $\varphi_1(w)$ for each node $w \in V$ and the sum of all coefficients are both bounded, then those terms are bounded by the top-k instance. 

% For the first term, the sum of the coefficients is at most
% \begin{align*}
%     \sum_{\substack{u \in U, uv \in \varphi_4(u) \\ w = \mathrm{arg\max}_{w\in \{u,v\}}d(w)}}\frac{1}{d(w)} \leq \sum_{\substack{u \in U, uv \in \varphi_4(u)}}\frac{1}{d(u)}  \leq \sum_{u \in U} 1 = k
% \end{align*}
% Besides, we can rewrite the first term as 
% \begin{align*}
% &\sum_{\substack{u \in U, uv \in \varphi_4(u) \\ w = \mathrm{arg\max}_{w\in \{u,v\}}d(w)}}\frac{|\varphi_1(w)| + |\varphi_3(w)|}{d(w)}
% = \sum_{\substack{u \in V, d(u) \geq d(v), \\ uv \in \varphi_4(u), u \in U \\ or (v, u) \in \varphi_4(v), v \in U}} \frac{|\varphi_1(u)| + |\varphi_3(u)|}{d(u)} 
% % &\leq \sum_{\substack{u \in V, d(u) \geq d(v), \\ uv \in \varphi_4(u), u \in U}} \frac{|\varphi_1(u)| + |\varphi_3(u)|}{d(u)} + \sum_{\substack{u \in V, d(u) \geq d(v) \\ (v, u) \in \varphi_4(v), v \in U}} \frac{|\varphi_1(u)| + |\varphi_3(u)|}{d(u)}
% \end{align*}
% For any $u\in V$, the coefficient is at most 
% \begin{align*}
%  \sum_{\substack{u \in V, d(u) \geq d(v), \\ uv \in \varphi_4(u), u \in U \\ or (v, u) \in \varphi_4(v), v \in U}} \frac{1}{d(u)} \leq \sum_{\substack{u \in V, d(u) \geq d(v), \\ uv \in \varphi_4(u), u \in U}} \frac{1}{d(u)} + \sum_{\substack{u \in V, d(u) \geq d(v) \\ (v, u) \in \varphi_4(v), v \in U}} \frac{1}{d(u)} = 2
% \end{align*}
% Therefore, for the first term, we have 
% \begin{align*}
%     \sum_{\substack{u \in U, uv \in \varphi_4(u) \\ w = \mathrm{arg\max}_{w\in \{u,v\}}d(w)}}\frac{|\varphi_1(w)| + |\varphi_3(w)|}{d(w)} \leq 2 \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}|\varphi_1(w)| + 2 \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}|\varphi_3(w)|
% \end{align*}

% For the second term, we have 
% \begin{align*}
%     &\sum_{\substack{u \in U, uv \in \varphi_4(u) \\ w = \mathrm{arg\max}_{w\in \{u,v\}}d(w)}} \frac{|\varphi_4(w)| - |N_H(u) \cap N_H(v)|}{d(w)} \\ &= \sum_{\substack{u \in U, uv \in \varphi_4(u) \\ w = \mathrm{arg\max}_{w\in \{u,v\}} d(w) \\ \Tilde{w} \in \{ u, v\} / \{ w \}}} \frac{|\varphi_4(w)| - |N_H(w) \cap N_H(\Tilde{w})|}{d(w)} \\
%     &\leq \sum_{\substack{u \in U, uv \in \varphi_4(u) \\ w = \mathrm{arg\max}_{w\in \{u,v\}} d(w) \\ \Tilde{w} \in \{ u, v\} / \{ w \}}} \frac{|\varphi_1(\Tilde{w})| + \cost^{-}_{\mathcal{C}}}(\Tilde{w})}{d(w)}
% \end{align*}
% Again, the sum of the coefficients is 
% \begin{align*}
%     \sum_{\substack{u \in U, uv \in \varphi_4(u) \\ w = \mathrm{arg\max}_{w\in \{u,v\}} d(w)}} \frac{1}{d(w)} \leq \sum_{\substack{u \in U, uv \in \varphi_4(u) }} \frac{1}{d(u)} \leq \sum_{u \in U} 1 = k
% \end{align*}
% We rewrite the second term as 
% \begin{align*}
%     \sum_{\substack{u \in U, uv \in \varphi_4(u) \\ w = \mathrm{arg\max}_{w\in \{u,v\}} d(w) \\ \Tilde{w} \in \{ u, v\} / \{ w \}}} \frac{|\varphi_1(\Tilde{w})| + \cost^{-}_{\mathcal{C}}}(\Tilde{w})}{d(w)} = \sum_{\substack{u \in V, d(u) \leq d(v), \\ uv \in \varphi_4(u), u \in U \\ or (v, u) \in \varphi_4(v), v \in U}} \frac{|\varphi_1(u)| + \cost^{-}_{\mathcal{C}}}(u)}{d(v)} 
% \end{align*}
% and the coefficient for each $u\in V$ is at most 
% \begin{align*}
%  \sum_{\substack{u \in V, d(u) \leq d(v), \\ uv \in \varphi_4(u), u \in U \\ or (v, u) \in \varphi_4(v), v \in U}} \frac{1}{d(v)} \leq \sum_{\substack{u \in V, d(u) \geq d(v), \\ uv \in \varphi_4(u), u \in U}} \frac{1}{d(v)} + \sum_{\substack{u \in V, d(u) \geq d(v) \\ (v, u) \in \varphi_4(v), v \in U}} \frac{1}{d(v)} = 2
% \end{align*}

% so the second term can be bounded by 
% \begin{align*}
%     &\sum_{\substack{u \in U, uv \in \varphi_4(u) \\ w = \mathrm{arg\max}_{w\in \{u,v\}} d(w) \\ \Tilde{w} \in \{ u, v\} / \{ w \}}} \frac{|\varphi_1(\Tilde{w})| + \cost^{-}_{\mathcal{C}}}(\Tilde{w})}{d(w)} \\ \leq& 2 \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}|\varphi_1(w)| + 2 \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}\cost^{-}_{\mathcal{C}}}(w)
% \end{align*}
% Combining together, we have 
% \begin{align*}
%     &\sum_{u \in U, uv \in \varphi_4(u)} x_{uv} \\
%     &\leq 2 \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}|\varphi_1(w)| + 4\cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}|\varphi_1(w)| + 2\cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}\cost^{-}_{\mathcal{C}}}(w) \\
%     &\leq 2\cost^k_G(\mathcal{C}) + 4 \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}|\varphi_1(w)|
% \end{align*}
% and 
% \begin{align*}
%     \sum_{u \in U} y^{+}(u)
%     &\leq \sum_{u \in U} |\varphi_1(u)| + \sum_{u \in U} |\varphi_3(u)| + \sum_{u \in U, uv \in \varphi_4(u)} x_{uv} \\
%     &\leq 3\cost^k_G(\mathcal{C}) + 5 \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}|\varphi_1(w)| \\
%     &\leq (3 + \frac{10}{\beta}) \cost^k_G(\mathcal{C})
% \end{align*}
% \end{proof}



\begin{lemma}
%For any graph $G$, let $x_{uv}$ be the output by Algorithm \ref{alg:pre-clusteringlp}. Given a clustering $\mathcal{C}$, any integer $k$ (s.t. $1\le k\le n$),  any subset $U \subset V$ such that $|U| = k$. Then, 
%\begin{align*}
    %&\sum_{u \in U} y^{-}(u) \leq \frac{2\beta - \beta^2}{(1 - \beta)^2} \cost^k_G(\mathcal{C}) 
%\end{align*}
    $f_6 \leq \frac2\beta \cdot \cost^k_\calC$.
\end{lemma}
\begin{proof}
We have 
% \begin{align*}
%     1 - x_{uv} &= \frac{|N_{H}(u) \cap N_{H}(v)|}{M_{uv}}.
% \end{align*}
%
%  Then we can bound $\sum_{u \in U} y^{-}(u)$ using $\varphi_5$, $\varphi_6$. 
% \begin{align*}
%     \sum_{u \in U} y^{-}(u) &= \sum_{u \in U} \big( \sum_{uv \in \varphi_5(u)} (1 - x_{uv}) + \sum_{uv \in \varphi_6(u)} (1 - x_{uv}) \big) \\
%     &\leq \sum_{u \in U} |\varphi_5(u)| + \sum_{u \in U, uv \in \varphi_6(u)} (1 - x_{uv})
% \end{align*}
% We have to bound $\sum_{u \in U, uv \in \varphi_6(u)} ( 1- x_{uv})$, 
%
% Since for any $uv \in \varphi_6(u)$, we know there exists a node $w \in N_{H}(u) \cap N_{H}(v)$. From fact 3.2 of \cite{cohen2021correlation}, we know that $(1 - 3\beta) \leq d(u) \leq \frac{d(v)}{1-3\beta}$ and $|N_{G}(u) \cap N_{G}(v)| \geq (1 - 3\beta) \mathrm{\max}(d(u), d(v))$.
%
%
...
\end{proof}


{\color{gray}
We have 2 cases for $w$, when $C(u) = \mathcal{C}(w)$. For each $uv \in \varphi_6(u)$, so $C(v) \not= \mathcal{C}(w)$. Each $v \in N_H(w)$ with $uv \in $ will contribute 1 disagreement for $w$, we have 
\begin{align*}
    \sum_{\substack{u \in N_{H}(w) \cap U \\v\in N_{H}(w), uv \in \varphi_6(u)}} \frac{1}{\mathrm{\max}(d(u), d(v))} \leq \sum_{\substack{u \in N_{H}(w) \\ u \in U}} \frac{\cost^{+}_{\mathcal{C}}(w)}{d(u)}
\end{align*}
When $C(u) \not= \mathcal{C}(w)$, since $w \in N_H(u)$, so $|N_G(u) \cap N_G(w)| \geq (1 - \beta) \cdot \max(d(u), d(w))$. we know that $\cost^{+}_{\mathcal{C}}(w) + \cost^{+}_{\mathcal{C}}(u) \geq |N_G(u) \cap N_G(w)| \geq (1 - \beta) \cdot \max(d(u), d(w))$ and 
\begin{align*}
    \sum_{\substack{u \in N_{H}(w) \cap U \\v\in N_{H}(w), uv \in \varphi_6(u)}} \frac{1}{\mathrm{\max}(d(u), d(v))} 
    &\leq \sum_{\substack{u \in N_{H}(w) \\ u \in U}} \frac{|N_H(w) \setminus N_H(u)|}{d(u)} \leq
    \sum_{\substack{u \in N_{H}(w) \\ u \in U}} \frac{\beta \max(d(u), d(w))}{d(u)}  \\
    &\leq \sum_{\substack{u \in N_{H}(w) \\ u \in U}} \frac{\beta}{1-\beta} \cdot \frac{\cost^{+}_{\mathcal{C}}(w) + \cost^{+}_{\mathcal{C}}(u)}{d(u)}
\end{align*}
When $\beta \geq 0.5$, we have 
\begin{align*}
    \sum_{u \in U, uv \in \varphi_6(u)} ( 1- x_{uv})
    &\leq \sum_{w \in V}\sum_{\substack{u \in N_{H}(w) \cap U \\v\in N_{H}(w), uv \in \varphi_6(u)}} \frac{1}{\mathrm{\max}(d(u), d(v))} \\
    &\leq \frac{\beta}{1-\beta} \cdot \sum_{w \in V, u \in N_H(w), u \in U} \frac{\cost^{+}_{\mathcal{C}}(w) + \cost^{+}_{\mathcal{C}}(u)}{d(u)} \\
    &\leq \frac{\beta}{1-\beta} \cdot \sum_{w \in V, u \in N_H(w), u \in U} \frac{\cost^{+}_{\mathcal{C}}(u)}{d(u)} + \frac{\beta}{1-\beta} \cdot \sum_{w \in V, u \in N_H(w), u \in U} \frac{\cost^{+}_{\mathcal{C}}(w)}{d(u)} \\
    &\leq \frac{\beta}{1-\beta} \cdot \sum_{u \in U} \cost^{+}_{\mathcal{C}}(u) + \frac{\beta}{1-\beta} \cdot \sum_{w \in V, u \in N_H(w), u \in U} \frac{\cost^{+}_{\mathcal{C}}(w)}{d(u)}
\end{align*}
For the second term, note that the sum of all coefficients for $\cost^{+}_{\mathcal{C}}(w)$ is 
\begin{align*}
    \sum_{w \in V, u \in N_H(w), u \in U} \frac{1}{d(u)} \leq \sum_{u \in U} \frac{d_H(u)}{d(u)} \leq k
\end{align*}
and for each $w\in V$, the coefficient is 
\begin{align*}
    \sum_{u \in N_H(w), u \in U} \frac{1}{d(u)} \leq \frac{d_H(w)}{d(u)} \leq \frac{1}{1-\beta}
\end{align*}
Therefore, we can bound the second term by 
\begin{align*}
    \frac{\beta}{1-\beta} \cdot \sum_{w \in V, u \in N_H(w), u \in U} \frac{\cost^{+}_{\mathcal{C}}(w)}{d(u)} \leq \frac{\beta}{(1-\beta)^2} \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}\cost^{+}_{\mathcal{C}}(w)
\end{align*}
Combining together, we have 
\begin{align*}
    \sum_{u \in U} y^{-}(u) &\leq \sum_{u \in U} |\varphi_5(u)| + \sum_{u \in U, uv \in \varphi_6(u)} (1 - x_{uv}) \\
    &\leq \sum_{u \in U} |\varphi_5(u)| + \frac{\beta}{1-\beta} \cdot \sum_{u \in U} \cost^{+}_{\mathcal{C}}(u) + \frac{\beta}{(1-\beta)^2} \cdot \mathrm{\max}_{U' \subset V, |U'| = k}\sum_{w \in U'}\cost^{+}_{\mathcal{C}}(w) \\
    &\leq \frac{2\beta - \beta^2}{(1 - \beta)^2} \cost^k_G(\mathcal{C}) 
\end{align*}}
